Track reconstruction as a service for collider physics

Optimizing charged-particle track reconstruction algorithms is crucial for efficient event reconstruction in Large Hadron Collider (LHC) experiments due to their significant computational demands. Existing track reconstruction algorithms have been adapted to run on massively parallel coprocessors, such as graphics processing units (GPUs), to reduce processing time. Nevertheless, challenges remain in fully harnessing the computational capacity of coprocessors in a scalable and non-disruptive manner. This paper proposes an inference-as-a-service approach for particle tracking in high energy physics experiments. To evaluate the efficacy of this approach, two distinct tracking algorithms are tested: Patatrack, a rule-based algorithm, and Exa$.$TrkX, a machine learning-based algorithm. The as-a-service implementations show enhanced GPU utilization and can process requests from multiple CPU cores concurrently without increasing per-request latency. The impact of data transfer is minimal and insignificant compared to running on local coprocessors. This approach greatly improves the computational efficiency of charged particle tracking, providing a solution to the computing challenges anticipated in the High-Luminosity LHC era.

==> scripts/scripts.tex <==
\usepackage{aas_macros}
\definecolor{Gray}{gray}{0.9}
\definecolor{Blue}{rgb}{0.88,1,1}
\definecolor{Red}{rgb}{1,0.88,0.88}
\newcolumntype{g}{>{\columncolor{Gray}}p}
\newcolumntype{b}{>{\columncolor{Blue}}p}
\newcolumntype{r}{>{\columncolor{Red}}p}
\usepackage{blindtext}
\usepackage{graphicx}

% Changing TOC Spacing to fit on one page
%\setlength{\cftbeforesecskip}{7pt}

\newenvironment{cititemize2}
{\begin{list}{$\bullet$}
        {\setlength{\topsep}{0pt}
         \setlength{\itemsep}{0pt}
         \setlength{\parsep}{0.25\parsep}
         \settowidth{\labelwidth}{$\bullet$}
         \setlength{\leftmargin}{1em}
}
}
{\end{list}}

\ifcsname ifdothebib\endcsname\else
  \expandafter\let\csname ifdothebib\expandafter\endcsname
                  \csname iffalse\endcsname
\fi



\newboolean{articletitles}
\setboolean{articletitles}{true} % False removes titles in references

\newboolean{uprightparticles}
\setboolean{uprightparticles}{false} %True for upright particle symbols

\newboolean{inbibliography}
\setboolean{inbibliography}{false} %True once you enter the bibliography


%\setlist{
%itemsep=1pt,
%partopsep=1pt,
%parsep=1pt}

% Figure spacing
\setlength{\textfloatsep}{8pt plus 2pt minus 2pt}
\setlength{\abovecaptionskip}{6pt}

%\sectionfont{\large}
%\subsectionfont{\normalize}

% Simple spacing
\titlespacing%
{\section}%
{0pt}% Left spacing
{3pt plus 2pt minus 2pt}% Before spacing
{3pt plus 2pt minus 2pt}% After spacing


\titlespacing%
{\subsection}%
{0pt}% Left spacing
{2pt plus 2pt minus 2pt}% Before spacing
{1pt plus 2pt minus 2pt}% After spacing

\titlespacing%
{\subsubsection}%
{0pt}% Left spacing
{2pt plus 2pt minus 2pt}% Before spacing
{1pt plus 2pt minus 2pt}% After spacing

% Inline subsections
%\titleformat{\subsection}[runin]
%{\normalfont\normalsize\bfseries}{\thesubsection}{1em}{}[: ]

% Inline subsubsections
%\titleformat{\subsubsection}[runin]
%{\normalfont\normalsize\bfseries}{\thesubsubsection}{1em}{}[: ]


\definecolor{mwcolor}{rgb}{0, 0.6, 0}
\definecolor{nsfcolor}{rgb}{0.2, 0.6, 0.6}
\definecolor{cambridgered}{RGB}{163,31,52}
\definecolor{cambridgegray}{rgb}{0.6,0.6,0.6}
\definecolor{cambridgegray2}{rgb}{0.4,0.4,0.4}


\acrodef{AI}{artificial intelligence}
\acrodef{DL}{deep learning}
\acrodef{CNN}{convolutional neural network}
\acrodef{CNN}{convolutional neural network}
\acrodef{RNN}{recurrent neural network}
\acrodef{GNN}{graph neural network}
\acrodef{GDL}{geometric deep learning methods}
\acrodef{NN}{neural network}
\acrodef{ML}{machine learning}
\acrodef{FML}{Fast Machine Learning}
\acrodef{SM}{standard model}
\acrodef{CMS}{The Compact Muon Solenoid}
\acrodef{QCD}{quantum chromodynamics}
\acrodef{LHC}{CERN Large Hadron Collider}
\acrodef{HL-LHC}{High-Luminosity LHC}
\acrodef{QFT}{quantum field theory}
\acrodef{IRC}{infrared and collinear}
\acrodef{EFN}{Energy Flow Network}
\acrodef{EMD}{earth mover's distance}
\acrodef{HPC}{high-performance computing}
\acrodef{A3D3}{Accelerated AI Algorithms for Data-Driven Discovery}
\acrodef{ASAML}{Advancing Science with Accelerated Machine Learning}
\acrodef{HDR}{Harnessing the Data Revolution}
\acrodef{LIGO}{Laser Interferometer Gravitational-Wave Observatory}
\acrodef{MMA}{multi-messenger astrophysics}
\acrodef{HEP}{high energy physics}
\acrodef{HLT}{high-level trigger}
\acrodef{L1T}{level-1 trigger}
\acrodef{BSM}{beyond the SM}
\acrodef{GW}{gravitational wave}
\acrodef{DUNE}{Deep Underground Neutrino Experiment}
\acrodef{LAr}{liquid argon}
\acrodef{TPC}{time-projection chamber}
\acrodef{ZTF}{Zwicky Transient Facility}

\acrodef{FPGA}{field-programmable gate array}
\acrodef{GPU}{graphics processing unit}
\acrodef{HLS}{high-level synthesis}
\acrodef{ASIC}{application-specific integrated circuit}
\acrodef{SONIC}{Services for Optimized Network Inference on Coprocessors}
\acrodef{L1DS}{Level 1 Data Scouting}
\acrodef{pp}{proton-proton}
\acrodef{URM}{underrepresented minority}

% Defining macros
\newcommand{\CAIFI}{CAIFI\xspace}
\newcommand{\ChiPhi}{{\large\textcolor{cambridgegray2}{X}\hspace{-0.75em}\textcolor{cambridgered}{$\Phi$}}\xspace}
\newcommand{\ChiPhiAlt}{\textcolor{cambridgegray2}{X}\textcolor{cambridgered}{$\Phi$}\xspace}


\renewcommand\thefootnote{\textit{\alph{footnote}}}
\newcommand{\hlsfml}{\texttt{hls4ml}\xspace}

\newcommand{\benedikt}[1]{{\textbf{\color{orange}{[Benedikt: #1]}}}}

\renewcommand{\paragraph}[1]{\noindent\emph{#1.}}
